DSANet: Dynamic Segment Aggregation Network for Video-Level Representation Learning

Long-range and short-range temporal modeling are two complementary and crucial aspects of video recognition. Most of the state-of-the-arts focus on short-range spatio-temporal modeling and then average multiple snippet-level predictions to yield the final video-level prediction. Thus, their video-level prediction does not consider spatio-temporal features of how video evolves along the temporal dimension. In this paper, we introduce a novel Dynamic Segment Aggregation (DSA) module to capture relationship among snippets. To be more specific, we attempt to generate a dynamic kernel for a convolutional operation to aggregate long-range temporal information among adjacent snippets adaptively. The DSA module is an efficient plug-and-play module and can be combined with the off-the-shelf clip-based models (i.e., TSM, I3D) to perform powerful long-range modeling with minimal overhead. The final video architecture, coined as DSANet. We conduct extensive experiments on several video recognition benchmarks (i.e., Mini-Kinetics-200, Kinetics-400, Something-Something V1 and ActivityNet) to show its superiority. Our proposed DSA module is shown to benefit various video recognition models significantly. For example, equipped with DSA modules, the top-1 accuracy of I3D ResNet-50 is improved from 74.9% to 78.2% on Kinetics-400. Codes are available at https://github.com/whwu95/DSANet.

==> intro.tex <==
\section{Introduction}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/teaser.pdf}
    \caption{
    The pipeline of our method for video recognition. One input video is divided into several segments and a short snippet is randomly sampled from each segment. Green trapezoids denote the snippet-level spatio-temporal networks (\emph{e.g.}, I3D, TSM) which share parameters on all snippets. DSA module can be easily inserted into the networks to capture long-range temporal structure.
    }
    \label{fig:overview}
\end{figure} 

% background of video recognition
With the rapid development of the Internet and mobile devices, video data has exploded over the past years. Video action recognition, as a fundamental problem in video analytics, has become one of the most active research topics. 

Previous methods have obtained noticeable improvements for video recognition.
3D CNNs are intuitive spatio-temporal networks and natural extension from their 2D counterparts, which directly tackle 3D volumetric video data~\cite{c3d,i3d}. However, the heavy computational cost of 3D CNNs limits its application. Recent studies have shown that factorizing 3D convolutional kernel into spatial (\emph{e.g.}, 1\x3\x3) and temporal components (\emph{e.g.}, 3\x1\x1) is preferable to reduce complexity as well as boost accuracy, \emph{e.g.}, P3D~\cite{p3d}, R(2+1)D~\cite{r2+1d}, Nonlocal+I3D~\cite{nonlocal}, SlowFast~\cite{slowfast}, \emph{etc}. 
In practice, however, compared with their 2D counterparts, the increased computational cost cannot be ignored.
To capture temporal information with reasonable computational cost, the other alternative 2D CNN based architectures are developed \emph{i.e.,} TSM~\cite{tsm}, TEI~\cite{teinet}, TEA~\cite{li2020tea}, MVFNet~\cite{wu2020MVFNet}, \emph{etc}. 
Temporal Shift Module (TSM)~\cite{tsm} is the representative 2D-based model, which achieves a good trade-off between performance and complexity meanwhile introduces zero FLOPs for the 2D CNN backbone. 
  
However, the above architectures, both based on 2D CNN and 3D CNN, are mainly designed to learn short-range spatio-temporal representation (snippet-level) instead of long-range representation (video-level).
Specifically, during training, these snippet-level methods sample sub-frames (4 frames, 8 frames or 16 frames) from a random snippet of the original video.
While for inference, they uniformly sample multiple short snippets from a video and compute the classification scores for all snippets individually and the final prediction is just the average voting from the snippet-level predictions.
Thus, these clip-based models take no account of modeling long-range temporal structure due to the limited observation of only a single snippet.
Also, simply averaging the prediction scores of all snippets could yield a sub-optimal solution during inference.

%video-level method
To alleviate the problem mentioned above, Temporal Segment Network~\cite{tsn} provides a simple framework to perform video-level learning, which just simply fuses snippet-level predictions. Lately, V4D~\cite{zhang2020v4d} presents an intuitive 4D convolutional operation to capture inter-clip interaction, which is a natural extension of enhancing the representation of the original clip-based 3D CNNs. However, TSN fails on capturing the finer temporal structure, (\emph{e.g.}, the temporal pattern of the ordering of features), and V4D causes high computational cost compared with the TSN-equipped counterpart and might lack the ability to describe the dynamics by simply employing a fixed number of video invariant kernels. This inspires us to focus on designing a temporal module, which keeps both advantages of high efficiency and strong flexibility of capturing long-range temporal structure.

% our method
In this paper, we creatively introduce a module to adaptively aggregate the features of multiple snippets, namely \emph{\textbf{D}ynamic \textbf{S}egment \textbf{A}ggregation Module} (\textbf{DSA} Module). 
Figure~\ref{fig:overview} illustrates the pipeline of our solution, DSA module is a novel generic module that can be easily plugged into the existing clip-based networks (\emph{e.g.,} TSM~\cite{tsm}, I3D~\cite{i3d}) to perform long-range modeling with the ignorable cost. 
Briefly, the DSA module firstly gets global context information from features of all snippets, then it utilizes the contextual view to learn the weight of aggregation in a channel-wise convolution manner.
Thus, DSA module can capture relation-ship among snippets via dynamic fusion along snippet dimension.
To make this module more efficient, we separate the features across the channel dimension. One keeps the original activation and the other performs dynamic segment aggregation separately followed by a concatenation operation.
In this way, DSA only introduces a bit more FLOPs which is close to zero, while bringing remarkable improvement. 
In practice, we integrate the DSA module into the existing spatio-temporal block (\emph{e.g.}, TSM block, I3D block) to form our DSANet.

% effectiveness
We identify the effectiveness of the proposed DSA module via comprehensive ablations. Extensive experimental results on multiple well-known datasets, including Mini-Kinetics-200~\cite{s3d}, Kinetics-400 \cite{kay2017kinetics}, Something-Something V1 \cite{sth-sth} and ActivityNet-v1.3 \cite{caba2015activitynet} show the superiority of our solution. All of these prove DSA boosts the performance over its snippet-level counterpart.
Overall, our major contributions are summarized as follows:

% contributions
\begin{itemize}
    \item Instead of snippet-level temporal modeling, we propose to exploit an effective and efficient video-level framework for learning video representation. To tackle this, the proposed DSA module provides a novel mechanism to adaptively aggregate snippet-level features.
    \item The DSA module works in a plug-and-play way and can be easily integrated into existing snippet-level methods. Without any bells and whistles, the DSA module brings consistent improvements when combined with both 2D CNN-based and 3D CNN-based methods (\emph{e.g.}, TSM, I3D, \emph{etc}).
    \item Extensive experiments on four public benchmark datasets demonstrate that the proposed DSA obtain an evident improvement over previous long-range temporal modeling methods with a minimal computational cost.
    
\end{itemize}
